CutClaw: Agentic Hours-Long Video Editing via Music Synchronization

Editing the video content with audio alignment forms a digital human-made art in current social media. However, the time-consuming and repetitive nature of manual video editing has long been a challenge for filmmakers and professional content creators alike. In this paper, we introduce CutClaw, an autonomous multi-agent framework designed to edit hours-long raw footage into meaningful short videos that leverages the capabilities of multiple Multimodal Language Models~(MLLMs) as an agent system. It produces videos with synchronized music, followed by instructions, and a visually appealing appearance. In detail, our approach begins by employing a hierarchical multimodal decomposition that captures both fine-grained details and global structures across visual and audio footage. Then, to ensure narrative consistency, a Playwriter Agent orchestrates the whole storytelling flow and structures the long-term narrative, anchoring visual scenes to musical shifts. Finally, to construct a short edited video, Editor and Reviewer Agents collaboratively optimize the final cut via selecting fine-grained visual content based on rigorous aesthetic and semantic criteria. We conduct detailed experiments to demonstrate that CutClaw significantly outperforms state-of-the-art baselines in generating high-quality, rhythm-aligned videos. The code is available at: https://github.com/GVCLab/CutClaw.

==> vis/fig/Playwriter/Playwriter.tex <==
\begin{figure*}[t]
\centering
  \includegraphics[width=\columnwidth]{vis/fig/Playwriter/Plyawriter.pdf}
  \vspace{-3em}
    \caption{\textbf{\textit{The workflow of Playwriter}}. Playwriter generate the whole storyline according to the input, and gives the detailed shot plan of each specific shot of music.}
  \label{fig:playwriter}
  \vspace{-1em}
\end{figure*}

==> vis/fig/video/video.tex <==
\begin{figure}[t]
\centering
  \includegraphics[height=1\textwidth]{vis/fig/video/VideoV3.pdf}
  \vspace{-1.5em}
  \caption{\textbf{\textit{Video Shots Aggregation}}. We first perform shot detection on the entire video and conduct a caption for a detailed understanding. Then, we use an LLM to aggregate similar content for a scene-level description.}
  \label{fig:video}
  \vspace{-1em}
\end{figure}

==> vis/table/benchmark_details.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Summary of the Proposed Benchmark Dataset and Experimental Setup.} Our benchmark emphasizes long-form source retrieval and diverse narrative complexities.}
\label{tab:benchmark_overview}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lp{1.5cm}p{5.5cm}p{5.5cm}}
\toprule
\textbf{Component} & \textbf{Quantity} & \textbf{Details} & \textbf{Role \& Challenge} \\
\midrule
\textbf{Visual Sources} & 10 Videos & \textbf{Total Duration:} $\approx$ 20 hours \newline \textbf{Total Shots:} $\approx$ xxx  \newline \textbf{Types:} 5 Movies + 5 Vlogs & Tests retrieval from large-scale, different scenarios. \\
\midrule
\textbf{Audio Sources} & 10 Tracks & \textbf{Genres:} Orchestral, Pop, Rock, Lo-fi, etc. \newline \textbf{Structure:} Diverse (Verse-Chorus / Linear) & Tests beat detection accuracy and structural narrative alignment across genres. \\
\midrule
\textbf{Instruction} & 20 Cases & \textbf{Levels:} 2 Levels of Complexity \newline (1. Object-centric, 2. Specific Narrowtive) \newline \textbf{Length:} 3 Levels \newline (1. 15s(several keypoints), 2. 1min(one structure), 3mins(whole music)) & Tests capability to handle instructions ranging from concrete queries to abstract storytelling. \\
\bottomrule
\end{tabular}%
}
\end{table*}
